Computational Complexity versus Statistical Performance on Sparse Recovery Problems

We show that several classical quantities controlling compressed sensing performance directly match classical parameters controlling algorithmic complexity. We first describe linearly convergent restart schemes on first-order methods solving a broad range of compressed sensing problems, where sharpness at the optimum controls convergence speed. We show that for sparse recovery problems, this sharpness can be written as a condition number, given by the ratio between true signal sparsity and the largest signal size that can be recovered by the observation matrix. In a similar vein, Renegar's condition number is a data-driven complexity measure for convex programs, generalizing classical condition numbers for linear systems. We show that for a broad class of compressed sensing problems, the worst case value of this algorithmic complexity measure taken over all signals matches the restricted singular value of the observation matrix which controls robust recovery performance. Overall, this means in both cases that, in compressed sensing problems, a single parameter directly controls both computational complexity and recovery performance. Numerical experiments illustrate these points using several classical algorithms.

==> sections/block_to_dispose.tex <==
\subsection{Optimization complexity and oversampling ratio}\label{s:oversampling}
If \eqref{def:nsp} is satisfied at a given order $s$ it is naturally also true at any $s'\leq s$. However the constant, and therefore the speed of convergence may change. Here we show that this constant actually depends on the ratio of the maximal order at which $A$ satisfies \eqref{def:nsp} and the sparsity of the signal that is decoded.

In that purpose we give a more concrete geometric meaning to the constant $\alpha$ in~\eqref{def:nsp} by connecting it with the diameter of a section of the $\ell_1$ ball by the null space of the matrix $A$ (see e.g. \citet{Kash07} for more details).

\begin{lemma}\label{lem:diam}
	Given a matrix $A\in\reals^{n \times p}$, denote
	\[
	\frac{1}{2}\diam(B_1^p \cap \Null(A))  = \sup_{\substack{Az=0\\\|z\|_1\leq 1}} \|z\|_2,
	\]
	the radius of the section of the $\ell_1$ ball $B_1^p$ by the null space of the matrix $A$ and 
	\BEQ\label{eq:s_A}
	s_A  = 1/\diam(B_1^p \cap \Null(A))^2,
	\EEQ
	a recovery threshold.
	Then $A$ satisfies NSP at any order $s < s_A$ with constant
	\BEQ\label{eq:alpha_recovery_threshold}
	\alpha = 2\sqrt{s_A/s} -1 >1.
	\EEQ
\end{lemma}
\begin{proof}
	For any $z\in\Null(A)$ and support set $S$ with $\Card(S)\leq s$, using equivalence of norms and definition of the radius,
	\[
	\|z_S\|_1 \leq \sqrt{s} ~\|z\|_2 \leq \frac{1}{2}\sqrt{\frac{s}{s_A}}~ \|z\|_1 = \frac{1}{2}\sqrt{\frac{s}{s_A}}~(\|z_S\|+\|z_{S^c}\|),
	\]
	which means, as $s <s_A$,
	\[
	\|z_{S^c}\|_1\geq (2\sqrt{s_A/s} -1 )\|z_S\|_1,
	\]
	hence the desired result.
\end{proof}

With $s_A$ defined in \eqref{eq:s_A}, for any original signals of sparsity $s <s_A$, sharpness bound~\eqref{eq:sharpness} reads then
\[
\|x\|_1-\|x^*\|_1 \geq \gamma \|x-x^*\|_1
\]
with $\gamma = \frac{\alpha-1}{\alpha+1} = 1-\sqrt{s/s_A}>0$.
The optimal restart scheme defined in Proposition~\ref{prop:complex-l1} has then complexity
\[
\|\hat y\|_1-\|x^*\|_1 \leq \exp\left( -\left(1-\sqrt{s/s_A} \right)\frac{e}{ 2\sqrt{p}}  N  \right) \epsilon_0.
\]
It means that for a given recovery threshold $s_A$, the sparser the signal, the faster the algorithm. 

Precise estimates of the diameter of random sections of norm balls can be computed using classical results in geometric functional analysis. The low $M^*$ estimates of \citet{Pajo86} for example show that when $E\subset \reals^p$ is a random subspace  of codimension $n$ (e.g. the null space of a random matrix~$A\in\reals^{n\times p}$), then
% VR: Precise what is the randomness for clean prop !
\[
\diam(B_1^p \cap E)\leq c \sqrt{\frac{\log p}{n}},
\]
with high probability, where $c>0$ is an absolute constant. This means that the recovery threshold $k_A$ satisfies
\[
s_A \geq n/(c^2\log p),
\]
with high probability and  leads to the following corollary.
\begin{corollary}
	For a random sampling matrix $A\in\reals^{n\times p}$ and any original signal $x^*$ of sparsity $s<n/(c^2\log p)$, with high probability, restart scheme \eqref{eq:restart} with optimal parameters defined in \eqref{eq:optimal_param} outputs a point $\hat y$ such that
	\[
	\|\hat y\|_1-\|x^*\|_1 \leq \exp\left( -\left(1-c\sqrt{\frac{s\log p}{n}} \right)\frac{e}{ 2\sqrt{p}}  N  \right) \epsilon_0,
	\]
	where $c$ is a universal constant and $N$ is the total number of iterations.
\end{corollary}
This means that the complexity of the optimization problem~\eqref{eq:l1-recov} is controlled by the oversampling ratio $n/s$. In other words while increasing the number of samples increases the time complexity of elementary operations of the algorithm, it increases its rate of convergence. 

==> sections/trash.tex <==
%VR Abstract
	We analyse sharp lower bounds on the optimum of sparse recovery problems. On one side we show that it ensures linear convergence of simple restart schemes. On the other side we link it to statistical measures of these problems such as the recovery threshold and the robustness to noisy observations. In particular we show that a single parameter, namely Renegar's condition number, controls both computational complexity and recovery performance. Overall this confirms taht recovery problems which are easier to solve from a statistical point of view (i.e. where more samples are available), are also easier to solve computationally.
	As a by product, we link null space constant and conically restricted eigenvalue, which could simplify analysis of classical sparse estimators. 
	Numerical experiments valid the performance of the restart scheme and show relevance of Renegar's condition number for sparse recovery problems.
	
	We show that several quantities controlling compressed sensing performance also directly control algorithmic complexity. We describe linearly convergent restart schemes solving a broad range of compressed sensing problems using first-order methods. The key term controlling convergence measures the sharpness of the optimum and can be interpreted as a condition number, computed as the ratio between the true signal sparsity and the maximum signal size that can be recovered by the observation matrix. In a similar vein, Renegar's condition number is a data-driven computational complexity measure for convex programs, generalizing classical condition numbers for linear systems. We provide evidence that for a broad class of compressed sensing problems, the worst case value of this algorithmic complexity measure taken over all signals matches the restricted eigenvalue of the observation matrix, which controls compressed sensing performance. This condition number also measures the robustness of the recovered solution with respect to a misspecification of the observation matrix $A$, a point rarely addressed by classical recovery results. Overall, this means that, in compressed sensing problems, a single parameter directly controls computational complexity and recovery performance.

% VR Intro
To relate the two aspects, we begin by studying the computational complexity of the exact sparse recovery problem and the approximation quality of the robust formulation. On one hand we show that the null space condition introduced by \citet{Cohe06} can be seen as a measure of sharpness on the optimum of the exact sparse recovery problem. This allows us to developp linearly convergent restart schemes whose rate depends on this sharpness. On the other hand we recall that approximation quality of the robust version is controlled by conically restricted singular values introduced by \citet{Bick07}. By linking null space propert constant and conically restricted singular values, we conclude that a single quantity controls both the linear rate of the restart scheme and the sensibility to noise of the robust problem. 

We detail concrete consequences of our results for random sensing operators showing that the more samples, the sharper the problem an so the faster the convergence for the exact recovery problem. In other words more observations not only increase the decoding performance but also decrease the computationnal complexity.

The key parameter revealed by our analysis is Renegar's condition number, a well-known data-driven complexity measure for convex conic linear systems. Its impact on computational aspects of recovery problems go beyond our restart scheme. What we show is that it matches the conically restricted singular values. This means that a single parameter controls both computational complexity and statistical performance. 

Finally we provide numerical experiments, first to valid the efficiency of our restart scheme, then to illustrate the relevance of Renegar's condition number for controlling both computational and statistical aspects.

Following recent results in optimization \citep{Bolt07}, we study sharp lower bounds on the optimum of exact sparse recovery problems. This sharpness ensure linear convergence of simple restart schemes, similar as ones developed by \citet{Roul17} or \citet{Gilp12}, that we present in Section~\ref{s:sharp}. This sharpness crucially depends on the null space property introduced by \citet{Cohe06} whose statistical aspects are explored in Section~\ref{s:renegar}. This shows first, that the more samples, the easier the problem on both computational and statistical point of view. Then this highlights that one single parameter, Renegar's condition number (known as a measure of complexity of conic linear systems), controls both the sharpness (hence the computational complexity) and the robustness of the recovery problem when observations are affected by noise (that is its statistical performance). As a byproduct this links the null space constant to conically restricted eigenvalues introduced by \citet{Bick07}, a result that could simplify calssical statistical analysis of estimators such as LASSO.
While first sections focus on the $\ell_1$ case for the sake of clarity, we extend our results to general sparisity recovery problems (when $x^*$ is a block-sparse vector or a low-rank matrix) in Section~\ref{s:beyond_l1}, using the framework of decomposable norms introduced by \citet{Nega09}. 
Finally numerical experiments in Section~\ref{s:numres} show the efficiency of our restart schemes for exact recovery and the relevance of Renegar's condition number to control both statistical and computational behavior of sparse recovery problems.

% VR Dual feasibility problem
 Remark that by a theorem of alternative, infeasibility of \eqref{eq:coneP} is equivalent to feasibility of the dual problem
\BEQ
\label{eq:coneD}
\tag{D\textsubscript{A,C}}
\BA{ll}
\mbox{find} & y\\
\mbox{s.t.} &  A^Ty \in \intr(C^\circ),
\EA
\EEQ
where $C^\circ$ is the polar cone of $C$.  

% VR NSP link with conic singular value
We are not aware of such links between null space property constant and minimal conically restricted singular values. This may simplify analysis of oracle estimates for robust recovery. For example definition of minimal conically restricted singular value by \citet{Bick07} differs slightly from the one of $\mu_s(A)$ given in~\eqref{def:mu_s_sparse} and reads
\[
\kappa(s,\alpha) = \inf_{\substack{S \in \llbracket 1, p \rrbracket \\ \Card(S) \leq s}} \inf_{\substack{\|x_{S^c}\|_1 \leq \alpha \|x_S\|_1 \\ \|x_S\|_2 =1}}  \|Ax\|_2 
\]
If positive it ensures stable recovery of LASSO and Dantzig estimators.
% VR: Best measure is compatibility as introduced by citet{Van_09} but let's keep it simple. 
% Remark first that the singular value is taken with respect to the $\ell_1$ norm not the Euclidean one and directly on the projection of the vector along coordinates lying in some support $S$. In our point of view this means defining distance to infeasiblity with respect to a different norm than the spectral one. 
Our definition requires $x$ to be on the unit sphere not only its projection on supports $S$ of cardinality $s$, a refined analysis may alleviate this difference.
But crucially positiveness of $\kappa(s,\alpha)$ (that ensures stable recovery) has two parameters. $\alpha$ encodes the largest constant such that \eqref{def:nsp} is satisfied. Our result shows that looking at $\kappa(s,1)$ may be sufficient to get positiveness of $\kappa(s,\alpha)$ for $\alpha$ larger than one. This may simplify recovery results by focusing only on the minimal conically restricted singular value $\mu_s(A)$.


